Geometric Random Edge

We show that a variant of the random-edge pivoting rule results in a strongly polynomial time simplex algorithm for linear programs $\max\{c^Tx \colon Ax\leq b\}$, whose constraint matrix $A$ satisfies a geometric property introduced by Brunsch and R\"oglin: The sine of the angle of a row of $A$ to a hyperplane spanned by $n-1$ other rows of $A$ is at least $\delta$. This property is a geometric generalization of $A$ being integral and all sub-determinants of $A$ being bounded by $\Delta$ in absolute value (since $\delta \geq 1/(\Delta^2 n)$). In particular, linear programs defined by totally unimodular matrices are captured in this famework ($\delta \geq 1/ n$) for which Dyer and Frieze previously described a strongly polynomial-time randomized algorithm. The number of pivots of the simplex algorithm is polynomial in the dimension and $1/\delta$ and independent of the number of constraints of the linear program. Our main result can be viewed as an algorithmic realization of the proof of small diameter for such polytopes by Bonifas et al., using the ideas of Dyer and Frieze.

==> S_and_boundary_picture_isoperimetric.tex <==
 \fill[  gray!30 ] ( 0 , 0 )
-- ( 0 , 0.50 )
-- ( 0.47 , 0.65 )
-- ( 0.47 , 0.15 )
-- ( 0 , 0 )
;  \fill[  gray!30 ] ( 0.47 , 0.15 )
-- ( 0.47 , 0.65 )
-- ( 0.94 , 0.81 )
-- ( 0.94 , 0.31 )
-- ( 0.47 , 0.15 )
;  \fill[  gray!30 ] ( 0.94 , 0.31 )
-- ( 0.94 , 0.81 )
-- ( 1.42 , 0.97 )
-- ( 1.42 , 0.47 )
-- ( 0.94 , 0.31 )
;  \fill[  gray!30 ] ( 1.42 , 0.47 )
-- ( 1.42 , 0.97 )
-- ( 1.89 , 1.13 )
-- ( 1.89 , 0.63 )
-- ( 1.42 , 0.47 )
;  \fill[  gray!30 ] ( 1.89 , 0.63 )
-- ( 1.89 , 1.13 )
-- ( 2.37 , 1.29 )
-- ( 2.37 , 0.79 )
-- ( 1.89 , 0.63 )
;  \fill[  gray!30 ] ( 2.37 , 0.79 )
-- ( 2.37 , 1.29 )
-- ( 2.84 , 1.44 )
-- ( 2.84 , 0.94 )
-- ( 2.37 , 0.79 )
;  \fill[  gray!30 ] ( 2.84 , 0.94 )
-- ( 2.84 , 1.44 )
-- ( 3.32 , 1.60 )
-- ( 3.32 , 1.10 )
-- ( 2.84 , 0.94 )
;  \fill[  gray!30 ] ( 3.32 , 1.10 )
-- ( 3.32 , 1.60 )
-- ( 3.79 , 1.76 )
-- ( 3.79 , 1.26 )
-- ( 3.32 , 1.10 )
;  \fill[  gray!30 ] ( 3.79 , 1.26 )
-- ( 3.79 , 1.76 )
-- ( 4.26 , 1.92 )
-- ( 4.26 , 1.42 )
-- ( 3.79 , 1.26 )
;  \fill[  gray!30 ] ( 4.26 , 1.42 )
-- ( 4.26 , 1.92 )
-- ( 4.74 , 2.08 )
-- ( 4.74 , 1.58 )
-- ( 4.26 , 1.42 )
;  \fill[  gray!30 ] ( 0 , 0.50 )
-- ( 0 , 1.00 )
-- ( 0.47 , 1.15 )
-- ( 0.47 , 0.65 )
-- ( 0 , 0.50 )
;  \fill[  gray!30 ] ( 0.47 , 0.65 )
-- ( 0.47 , 1.15 )
-- ( 0.94 , 1.31 )
-- ( 0.94 , 0.81 )
-- ( 0.47 , 0.65 )
;  \fill[  gray!30 ] ( 0.94 , 0.81 )
-- ( 0.94 , 1.31 )
-- ( 1.42 , 1.47 )
-- ( 1.42 , 0.97 )
-- ( 0.94 , 0.81 )
;  \fill[  gray!30 ] ( 1.42 , 0.97 )
-- ( 1.42 , 1.47 )
-- ( 1.89 , 1.63 )
-- ( 1.89 , 1.13 )
-- ( 1.42 , 0.97 )
;  \fill[  gray!30 ] ( 1.89 , 1.13 )
-- ( 1.89 , 1.63 )
-- ( 2.37 , 1.79 )
-- ( 2.37 , 1.29 )
-- ( 1.89 , 1.13 )
;  \fill[  gray!30 ] ( 2.37 , 1.29 )
-- ( 2.37 , 1.79 )
-- ( 2.84 , 1.94 )
-- ( 2.84 , 1.44 )
-- ( 2.37 , 1.29 )
;  \fill[  gray!30 ] ( 2.84 , 1.44 )
-- ( 2.84 , 1.94 )
-- ( 3.32 , 2.10 )
-- ( 3.32 , 1.60 )
-- ( 2.84 , 1.44 )
;  \fill[  gray!30 ] ( 3.32 , 1.60 )
-- ( 3.32 , 2.10 )
-- ( 3.79 , 2.26 )
-- ( 3.79 , 1.76 )
-- ( 3.32 , 1.60 )
;  \fill[  gray!30 ] ( 3.79 , 1.76 )
-- ( 3.79 , 2.26 )
-- ( 4.26 , 2.42 )
-- ( 4.26 , 1.92 )
-- ( 3.79 , 1.76 )
;  \fill[  gray!30 ] ( 0 , 1.00 )
-- ( 0 , 1.50 )
-- ( 0.47 , 1.65 )
-- ( 0.47 , 1.15 )
-- ( 0 , 1.00 )
;  \fill[  gray!30 ] ( 1.89 , 1.63 )
-- ( 1.89 , 2.13 )
-- ( 2.37 , 2.29 )
-- ( 2.37 , 1.79 )
-- ( 1.89 , 1.63 )
;  \fill[  gray!30 ] ( 2.37 , 1.79 )
-- ( 2.37 , 2.29 )
-- ( 2.84 , 2.44 )
-- ( 2.84 , 1.94 )
-- ( 2.37 , 1.79 )
;  \fill[  gray!30 ] ( 2.84 , 1.94 )
-- ( 2.84 , 2.44 )
-- ( 3.32 , 2.60 )
-- ( 3.32 , 2.10 )
-- ( 2.84 , 1.94 )
;  \fill[  gray!30 ] ( 1.89 , 2.13 )
-- ( 1.89 , 2.63 )
-- ( 2.37 , 2.79 )
-- ( 2.37 , 2.29 )
-- ( 1.89 , 2.13 )
;  \fill[  gray!30 ] ( 0 , 0 )
-- ( 0.47 , 0.15 )
-- ( 0.75 , -0.25 )
-- ( 0.27 , -0.41 )
-- ( 0 , 0 )
;  \fill[  gray!30 ] ( 0.27 , -0.41 )
-- ( 0.75 , -0.25 )
-- ( 1.02 , -0.67 )
-- ( 0.55 , -0.83 )
-- ( 0.27 , -0.41 )
;  \fill[  gray!30 ] ( 0.55 , -0.83 )
-- ( 1.02 , -0.67 )
-- ( 1.30 , -1.08 )
-- ( 0.83 , -1.24 )
-- ( 0.55 , -0.83 )
;  \fill[  gray!30 ] ( 0.47 , 0.15 )
-- ( 0.94 , 0.31 )
-- ( 1.22 , -0.09 )
-- ( 0.75 , -0.25 )
-- ( 0.47 , 0.15 )
;  \fill[  gray!30 ] ( 0.75 , -0.25 )
-- ( 1.22 , -0.09 )
-- ( 1.50 , -0.51 )
-- ( 1.02 , -0.67 )
-- ( 0.75 , -0.25 )
;  \fill[  gray!30 ] ( 1.02 , -0.67 )
-- ( 1.50 , -0.51 )
-- ( 1.78 , -0.93 )
-- ( 1.30 , -1.08 )
-- ( 1.02 , -0.67 )
;  \fill[  gray!30 ] ( 1.30 , -1.08 )
-- ( 1.78 , -0.93 )
-- ( 2.05 , -1.34 )
-- ( 1.58 , -1.50 )
-- ( 1.30 , -1.08 )
;  \fill[  gray!30 ] ( 1.58 , -1.50 )
-- ( 2.05 , -1.34 )
-- ( 2.33 , -1.76 )
-- ( 1.86 , -1.92 )
-- ( 1.58 , -1.50 )
;  \fill[  gray!30 ] ( 1.86 , -1.92 )
-- ( 2.33 , -1.76 )
-- ( 2.61 , -2.17 )
-- ( 2.13 , -2.33 )
-- ( 1.86 , -1.92 )
;  \fill[  gray!30 ] ( 0.94 , 0.31 )
-- ( 1.42 , 0.47 )
-- ( 1.70 , 0.05 )
-- ( 1.22 , -0.09 )
-- ( 0.94 , 0.31 )
;  \fill[  gray!30 ] ( 1.22 , -0.09 )
-- ( 1.70 , 0.05 )
-- ( 1.97 , -0.35 )
-- ( 1.50 , -0.51 )
-- ( 1.22 , -0.09 )
;  \fill[  gray!30 ] ( 1.50 , -0.51 )
-- ( 1.97 , -0.35 )
-- ( 2.25 , -0.77 )
-- ( 1.78 , -0.93 )
-- ( 1.50 , -0.51 )
;  \fill[  gray!30 ] ( 1.78 , -0.93 )
-- ( 2.25 , -0.77 )
-- ( 2.53 , -1.18 )
-- ( 2.05 , -1.34 )
-- ( 1.78 , -0.93 )
;  \fill[  gray!30 ] ( 2.05 , -1.34 )
-- ( 2.53 , -1.18 )
-- ( 2.80 , -1.60 )
-- ( 2.33 , -1.76 )
-- ( 2.05 , -1.34 )
;  \fill[  gray!30 ] ( 2.33 , -1.76 )
-- ( 2.80 , -1.60 )
-- ( 3.08 , -2.02 )
-- ( 2.61 , -2.17 )
-- ( 2.33 , -1.76 )
;  \fill[  gray!30 ] ( 1.42 , 0.47 )
-- ( 1.89 , 0.63 )
-- ( 2.17 , 0.21 )
-- ( 1.70 , 0.05 )
-- ( 1.42 , 0.47 )
;  \fill[  gray!30 ] ( 1.70 , 0.05 )
-- ( 2.17 , 0.21 )
-- ( 2.45 , -0.19 )
-- ( 1.97 , -0.35 )
-- ( 1.70 , 0.05 )
;  \fill[  gray!30 ] ( 1.97 , -0.35 )
-- ( 2.45 , -0.19 )
-- ( 2.72 , -0.61 )
-- ( 2.25 , -0.77 )
-- ( 1.97 , -0.35 )
;  \fill[  gray!30 ] ( 2.25 , -0.77 )
-- ( 2.72 , -0.61 )
-- ( 3.00 , -1.03 )
-- ( 2.53 , -1.18 )
-- ( 2.25 , -0.77 )
;  \fill[  gray!30 ] ( 2.53 , -1.18 )
-- ( 3.00 , -1.03 )
-- ( 3.28 , -1.44 )
-- ( 2.80 , -1.60 )
-- ( 2.53 , -1.18 )
;  \fill[  gray!30 ] ( 2.80 , -1.60 )
-- ( 3.28 , -1.44 )
-- ( 3.56 , -1.86 )
-- ( 3.08 , -2.02 )
-- ( 2.80 , -1.60 )
;  \fill[  gray!30 ] ( 1.89 , 0.63 )
-- ( 2.37 , 0.79 )
-- ( 2.64 , 0.37 )
-- ( 2.17 , 0.21 )
-- ( 1.89 , 0.63 )
;  \fill[  gray!30 ] ( 2.17 , 0.21 )
-- ( 2.64 , 0.37 )
-- ( 2.92 , -0.04 )
-- ( 2.45 , -0.19 )
-- ( 2.17 , 0.21 )
;  \fill[  gray!30 ] ( 2.45 , -0.19 )
-- ( 2.92 , -0.04 )
-- ( 3.20 , -0.45 )
-- ( 2.72 , -0.61 )
-- ( 2.45 , -0.19 )
;  \fill[  gray!30 ] ( 2.72 , -0.61 )
-- ( 3.20 , -0.45 )
-- ( 3.48 , -0.87 )
-- ( 3.00 , -1.03 )
-- ( 2.72 , -0.61 )
;  \fill[  gray!30 ] ( 3.00 , -1.03 )
-- ( 3.48 , -0.87 )
-- ( 3.75 , -1.28 )
-- ( 3.28 , -1.44 )
-- ( 3.00 , -1.03 )
;  \fill[  gray!30 ] ( 3.28 , -1.44 )
-- ( 3.75 , -1.28 )
-- ( 4.03 , -1.70 )
-- ( 3.56 , -1.86 )
-- ( 3.28 , -1.44 )
;  \fill[  gray!30 ] ( 2.37 , 0.79 )
-- ( 2.84 , 0.94 )
-- ( 3.12 , 0.53 )
-- ( 2.64 , 0.37 )
-- ( 2.37 , 0.79 )
;  \fill[  gray!30 ] ( 2.64 , 0.37 )
-- ( 3.12 , 0.53 )
-- ( 3.40 , 0.11 )
-- ( 2.92 , -0.04 )
-- ( 2.64 , 0.37 )
;  \fill[  gray!30 ] ( 2.92 , -0.04 )
-- ( 3.40 , 0.11 )
-- ( 3.67 , -0.29 )
-- ( 3.20 , -0.45 )
-- ( 2.92 , -0.04 )
;  \fill[  gray!30 ] ( 3.20 , -0.45 )
-- ( 3.67 , -0.29 )
-- ( 3.95 , -0.71 )
-- ( 3.48 , -0.87 )
-- ( 3.20 , -0.45 )
;  \fill[  gray!30 ] ( 3.48 , -0.87 )
-- ( 3.95 , -0.71 )
-- ( 4.23 , -1.13 )
-- ( 3.75 , -1.28 )
-- ( 3.48 , -0.87 )
;  \fill[  gray!30 ] ( 3.75 , -1.28 )
-- ( 4.23 , -1.13 )
-- ( 4.51 , -1.54 )
-- ( 4.03 , -1.70 )
-- ( 3.75 , -1.28 )
;  \fill[  gray!30 ] ( 4.03 , -1.70 )
-- ( 4.51 , -1.54 )
-- ( 4.78 , -1.96 )
-- ( 4.31 , -2.12 )
-- ( 4.03 , -1.70 )
;  \fill[  gray!30 ] ( 2.84 , 0.94 )
-- ( 3.32 , 1.10 )
-- ( 3.59 , 0.69 )
-- ( 3.12 , 0.53 )
-- ( 2.84 , 0.94 )
;  \fill[  gray!30 ] ( 3.12 , 0.53 )
-- ( 3.59 , 0.69 )
-- ( 3.87 , 0.27 )
-- ( 3.40 , 0.11 )
-- ( 3.12 , 0.53 )
;  \fill[  gray!30 ] ( 3.40 , 0.11 )
-- ( 3.87 , 0.27 )
-- ( 4.15 , -0.14 )
-- ( 3.67 , -0.29 )
-- ( 3.40 , 0.11 )
;  \fill[  gray!30 ] ( 4.23 , -1.13 )
-- ( 4.70 , -0.97 )
-- ( 4.98 , -1.38 )
-- ( 4.51 , -1.54 )
-- ( 4.23 , -1.13 )
;  \fill[  gray!30 ] ( 4.51 , -1.54 )
-- ( 4.98 , -1.38 )
-- ( 5.26 , -1.80 )
-- ( 4.78 , -1.96 )
-- ( 4.51 , -1.54 )
;  \fill[  gray!30 ] ( 3.32 , 1.10 )
-- ( 3.79 , 1.26 )
-- ( 4.07 , 0.84 )
-- ( 3.59 , 0.69 )
-- ( 3.32 , 1.10 )
;  \fill[  gray!30 ] ( 3.59 , 0.69 )
-- ( 4.07 , 0.84 )
-- ( 4.34 , 0.43 )
-- ( 3.87 , 0.27 )
-- ( 3.59 , 0.69 )
;  \fill[  gray!30 ] ( 4.70 , -0.97 )
-- ( 5.18 , -0.81 )
-- ( 5.45 , -1.23 )
-- ( 4.98 , -1.38 )
-- ( 4.70 , -0.97 )
;  \fill[  gray!30 ] ( 3.79 , 1.26 )
-- ( 4.26 , 1.42 )
-- ( 4.54 , 1.00 )
-- ( 4.07 , 0.84 )
-- ( 3.79 , 1.26 )
;  \fill[  gray!30 ] ( 5.18 , -0.81 )
-- ( 5.65 , -0.65 )
-- ( 5.93 , -1.07 )
-- ( 5.45 , -1.23 )
-- ( 5.18 , -0.81 )
;  \fill[  gray!30 ] ( 4.26 , 1.42 )
-- ( 4.74 , 1.58 )
-- ( 5.02 , 1.16 )
-- ( 4.54 , 1.00 )
-- ( 4.26 , 1.42 )
;  \fill[  gray!30 ] ( 4.54 , 1.00 )
-- ( 5.02 , 1.16 )
-- ( 5.29 , 0.74 )
-- ( 4.82 , 0.59 )
-- ( 4.54 , 1.00 )
;  \fill[  gray!30 ] ( 5.37 , -0.24 )
-- ( 5.85 , -0.08 )
-- ( 6.13 , -0.49 )
-- ( 5.65 , -0.65 )
-- ( 5.37 , -0.24 )
;  \fill[  gray!30 ] ( 5.65 , -0.65 )
-- ( 6.13 , -0.49 )
-- ( 6.40 , -0.91 )
-- ( 5.93 , -1.07 )
-- ( 5.65 , -0.65 )
;  \fill[  gray!30 ] ( 5.02 , 1.16 )
-- ( 5.49 , 1.32 )
-- ( 5.77 , 0.90 )
-- ( 5.29 , 0.74 )
-- ( 5.02 , 1.16 )
;  \fill[  gray!30 ] ( 5.29 , 0.74 )
-- ( 5.77 , 0.90 )
-- ( 6.04 , 0.49 )
-- ( 5.57 , 0.33 )
-- ( 5.29 , 0.74 )
;  \fill[  gray!30 ] ( 5.57 , 0.33 )
-- ( 6.04 , 0.49 )
-- ( 6.32 , 0.07 )
-- ( 5.85 , -0.08 )
-- ( 5.57 , 0.33 )
;  \fill[  gray!30 ] ( 5.85 , -0.08 )
-- ( 6.32 , 0.07 )
-- ( 6.60 , -0.34 )
-- ( 6.13 , -0.49 )
-- ( 5.85 , -0.08 )
;  \fill[  gray!30 ] ( 6.13 , -0.49 )
-- ( 6.60 , -0.34 )
-- ( 6.88 , -0.75 )
-- ( 6.40 , -0.91 )
-- ( 6.13 , -0.49 )
;  \fill[  gray!30 ] ( 5.77 , 0.90 )
-- ( 6.24 , 1.06 )
-- ( 6.52 , 0.64 )
-- ( 6.04 , 0.49 )
-- ( 5.77 , 0.90 )
;  \fill[  gray!30 ] ( 6.04 , 0.49 )
-- ( 6.52 , 0.64 )
-- ( 6.80 , 0.23 )
-- ( 6.32 , 0.07 )
-- ( 6.04 , 0.49 )
;  \fill[  gray!30 ] ( 0 , 0 )
-- ( 0.27 , -0.41 )
-- ( 0.09 , -0.88 )
-- ( -0.18 , -0.46 )
-- ( 0 , 0 )
;  \fill[  gray!30 ] ( -0.18 , -0.46 )
-- ( 0.09 , -0.88 )
-- ( -0.09 , -1.34 )
-- ( -0.37 , -0.92 )
-- ( -0.18 , -0.46 )
;  \fill[  gray!30 ] ( -0.37 , -0.92 )
-- ( -0.09 , -1.34 )
-- ( -0.27 , -1.80 )
-- ( -0.55 , -1.39 )
-- ( -0.37 , -0.92 )
;  \fill[  gray!30 ] ( -0.55 , -1.39 )
-- ( -0.27 , -1.80 )
-- ( -0.46 , -2.27 )
-- ( -0.74 , -1.85 )
-- ( -0.55 , -1.39 )
;  \fill[  gray!30 ] ( 0.27 , -0.41 )
-- ( 0.55 , -0.83 )
-- ( 0.36 , -1.29 )
-- ( 0.09 , -0.88 )
-- ( 0.27 , -0.41 )
;  \fill[  gray!30 ] ( 0.09 , -0.88 )
-- ( 0.36 , -1.29 )
-- ( 0.18 , -1.76 )
-- ( -0.09 , -1.34 )
-- ( 0.09 , -0.88 )
;  \fill[  gray!30 ] ( -0.09 , -1.34 )
-- ( 0.18 , -1.76 )
-- ( -0.00 , -2.22 )
-- ( -0.27 , -1.80 )
-- ( -0.09 , -1.34 )
;  \fill[  gray!30 ] ( 0.55 , -0.83 )
-- ( 0.83 , -1.24 )
-- ( 0.64 , -1.71 )
-- ( 0.36 , -1.29 )
-- ( 0.55 , -0.83 )
;  \fill[  gray!30 ] ( 0 , 0 )
-- ( -0.18 , -0.46 )
-- ( -0.60 , -0.18 )
-- ( -0.41 , 0.27 )
-- ( 0 , 0 )
;  \fill[  gray!30 ] ( -0.41 , 0.27 )
-- ( -0.60 , -0.18 )
-- ( -1.01 , 0.09 )
-- ( -0.83 , 0.55 )
-- ( -0.41 , 0.27 )
;  \fill[  gray!30 ] ( -0.83 , 0.55 )
-- ( -1.01 , 0.09 )
-- ( -1.43 , 0.36 )
-- ( -1.24 , 0.83 )
-- ( -0.83 , 0.55 )
;  \fill[  gray!30 ] ( -1.24 , 0.83 )
-- ( -1.43 , 0.36 )
-- ( -1.84 , 0.64 )
-- ( -1.66 , 1.10 )
-- ( -1.24 , 0.83 )
;  \fill[  gray!30 ] ( -3.32 , 2.21 )
-- ( -3.51 , 1.75 )
-- ( -3.92 , 2.03 )
-- ( -3.74 , 2.49 )
-- ( -3.32 , 2.21 )
;  \fill[  gray!30 ] ( -3.74 , 2.49 )
-- ( -3.92 , 2.03 )
-- ( -4.34 , 2.30 )
-- ( -4.16 , 2.77 )
-- ( -3.74 , 2.49 )
;  \fill[  gray!30 ] ( -4.16 , 2.77 )
-- ( -4.34 , 2.30 )
-- ( -4.76 , 2.58 )
-- ( -4.57 , 3.05 )
-- ( -4.16 , 2.77 )
;  \fill[  gray!30 ] ( -0.18 , -0.46 )
-- ( -0.37 , -0.92 )
-- ( -0.78 , -0.65 )
-- ( -0.60 , -0.18 )
-- ( -0.18 , -0.46 )
;  \fill[  gray!30 ] ( -0.60 , -0.18 )
-- ( -0.78 , -0.65 )
-- ( -1.20 , -0.37 )
-- ( -1.01 , 0.09 )
-- ( -0.60 , -0.18 )
;  \fill[  gray!30 ] ( -1.01 , 0.09 )
-- ( -1.20 , -0.37 )
-- ( -1.61 , -0.09 )
-- ( -1.43 , 0.36 )
-- ( -1.01 , 0.09 )
;  \fill[  gray!30 ] ( -1.43 , 0.36 )
-- ( -1.61 , -0.09 )
-- ( -2.03 , 0.18 )
-- ( -1.84 , 0.64 )
-- ( -1.43 , 0.36 )
;  \fill[  gray!30 ] ( -3.51 , 1.75 )
-- ( -3.69 , 1.29 )
-- ( -4.11 , 1.56 )
-- ( -3.92 , 2.03 )
-- ( -3.51 , 1.75 )
;  \fill[  gray!30 ] ( -3.92 , 2.03 )
-- ( -4.11 , 1.56 )
-- ( -4.53 , 1.84 )
-- ( -4.34 , 2.30 )
-- ( -3.92 , 2.03 )
;  \fill[  gray!30 ] ( -4.34 , 2.30 )
-- ( -4.53 , 1.84 )
-- ( -4.94 , 2.12 )
-- ( -4.76 , 2.58 )
-- ( -4.34 , 2.30 )
;  \fill[  gray!30 ] ( -0.37 , -0.92 )
-- ( -0.55 , -1.39 )
-- ( -0.97 , -1.11 )
-- ( -0.78 , -0.65 )
-- ( -0.37 , -0.92 )
;  \fill[  gray!30 ] ( -0.78 , -0.65 )
-- ( -0.97 , -1.11 )
-- ( -1.38 , -0.83 )
-- ( -1.20 , -0.37 )
-- ( -0.78 , -0.65 )
;  \fill[  gray!30 ] ( -1.20 , -0.37 )
-- ( -1.38 , -0.83 )
-- ( -1.80 , -0.56 )
-- ( -1.61 , -0.09 )
-- ( -1.20 , -0.37 )
;  \fill[  gray!30 ] ( -1.61 , -0.09 )
-- ( -1.80 , -0.56 )
-- ( -2.22 , -0.28 )
-- ( -2.03 , 0.18 )
-- ( -1.61 , -0.09 )
;  \fill[  gray!30 ] ( -3.69 , 1.29 )
-- ( -3.88 , 0.82 )
-- ( -4.30 , 1.10 )
-- ( -4.11 , 1.56 )
-- ( -3.69 , 1.29 )
;  \fill[  gray!30 ] ( -4.11 , 1.56 )
-- ( -4.30 , 1.10 )
-- ( -4.71 , 1.38 )
-- ( -4.53 , 1.84 )
-- ( -4.11 , 1.56 )
;  \fill[  gray!30 ] ( -4.53 , 1.84 )
-- ( -4.71 , 1.38 )
-- ( -5.13 , 1.65 )
-- ( -4.94 , 2.12 )
-- ( -4.53 , 1.84 )
;  \fill[  gray!30 ] ( -0.55 , -1.39 )
-- ( -0.74 , -1.85 )
-- ( -1.15 , -1.57 )
-- ( -0.97 , -1.11 )
-- ( -0.55 , -1.39 )
;  \fill[  gray!30 ] ( -0.97 , -1.11 )
-- ( -1.15 , -1.57 )
-- ( -1.57 , -1.30 )
-- ( -1.38 , -0.83 )
-- ( -0.97 , -1.11 )
;  \fill[  gray!30 ] ( -1.38 , -0.83 )
-- ( -1.57 , -1.30 )
-- ( -1.99 , -1.02 )
-- ( -1.80 , -0.56 )
-- ( -1.38 , -0.83 )
;  \fill[  gray!30 ] ( -4.30 , 1.10 )
-- ( -4.48 , 0.63 )
-- ( -4.90 , 0.91 )
-- ( -4.71 , 1.38 )
-- ( -4.30 , 1.10 )
;  \fill[  gray!30 ] ( -4.71 , 1.38 )
-- ( -4.90 , 0.91 )
-- ( -5.31 , 1.19 )
-- ( -5.13 , 1.65 )
-- ( -4.71 , 1.38 )
;  \fill[  gray!30 ] ( -1.15 , -1.57 )
-- ( -1.34 , -2.04 )
-- ( -1.76 , -1.76 )
-- ( -1.57 , -1.30 )
-- ( -1.15 , -1.57 )
;  \fill[  gray!30 ] ( 0 , 0 )
-- ( -0.41 , 0.27 )
-- ( -0.41 , 0.77 )
-- ( 0 , 0.50 )
-- ( 0 , 0 )
;  \fill[  gray!30 ] ( 0 , 0.50 )
-- ( -0.41 , 0.77 )
-- ( -0.41 , 1.27 )
-- ( 0 , 1.00 )
-- ( 0 , 0.50 )
;  \fill[  gray!30 ] ( 0 , 1.00 )
-- ( -0.41 , 1.27 )
-- ( -0.41 , 1.77 )
-- ( 0 , 1.50 )
-- ( 0 , 1.00 )
;  \fill[  gray!30 ] ( -0.41 , 0.27 )
-- ( -0.83 , 0.55 )
-- ( -0.83 , 1.05 )
-- ( -0.41 , 0.77 )
-- ( -0.41 , 0.27 )
;  \fill[  gray!30 ] ( -0.41 , 0.77 )
-- ( -0.83 , 1.05 )
-- ( -0.83 , 1.55 )
-- ( -0.41 , 1.27 )
-- ( -0.41 , 0.77 )
;  \fill[  gray!30 ] ( -0.41 , 1.27 )
-- ( -0.83 , 1.55 )
-- ( -0.83 , 2.05 )
-- ( -0.41 , 1.77 )
-- ( -0.41 , 1.27 )
;  \fill[  gray!30 ] ( -0.83 , 0.55 )
-- ( -1.24 , 0.83 )
-- ( -1.24 , 1.33 )
-- ( -0.83 , 1.05 )
-- ( -0.83 , 0.55 )
;  \fill[  gray!30 ] ( -0.83 , 1.05 )
-- ( -1.24 , 1.33 )
-- ( -1.24 , 1.83 )
-- ( -0.83 , 1.55 )
-- ( -0.83 , 1.05 )
;  \fill[  gray!30 ] ( -0.83 , 1.55 )
-- ( -1.24 , 1.83 )
-- ( -1.24 , 2.33 )
-- ( -0.83 , 2.05 )
-- ( -0.83 , 1.55 )
;  \fill[  gray!30 ] ( -1.24 , 0.83 )
-- ( -1.66 , 1.10 )
-- ( -1.66 , 1.60 )
-- ( -1.24 , 1.33 )
-- ( -1.24 , 0.83 )
;  \fill[  gray!30 ] ( -1.24 , 1.33 )
-- ( -1.66 , 1.60 )
-- ( -1.66 , 2.10 )
-- ( -1.24 , 1.83 )
-- ( -1.24 , 1.33 )
;  \fill[  gray!30 ] ( -3.32 , 2.21 )
-- ( -3.74 , 2.49 )
-- ( -3.74 , 2.99 )
-- ( -3.32 , 2.71 )
-- ( -3.32 , 2.21 )
;  \fill[  gray!30 ] ( -3.74 , 2.49 )
-- ( -4.16 , 2.77 )
-- ( -4.16 , 3.27 )
-- ( -3.74 , 2.99 )
-- ( -3.74 , 2.49 )
;  \fill[  gray!30 ] ( -4.16 , 2.77 )
-- ( -4.57 , 3.05 )
-- ( -4.57 , 3.55 )
-- ( -4.16 , 3.27 )
-- ( -4.16 , 2.77 )
;  \draw[  blue, line width = 1.5pt ] ( 4.26 , 1.92 )
-- ( 4.74 , 2.08 )
;  \draw[  blue, line width = 1.5pt ] ( 4.74 , 2.08 )
-- ( 4.74 , 1.58 )
;  \draw[  blue, line width = 1.5pt ] ( 0.47 , 1.15 )
-- ( 0.94 , 1.31 )
;  \draw[  blue, line width = 1.5pt ] ( 0.94 , 1.31 )
-- ( 1.42 , 1.47 )
;  \draw[  blue, line width = 1.5pt ] ( 1.42 , 1.47 )
-- ( 1.89 , 1.63 )
;  \draw[  blue, line width = 1.5pt ] ( 3.32 , 2.10 )
-- ( 3.79 , 2.26 )
;  \draw[  blue, line width = 1.5pt ] ( 3.79 , 2.26 )
-- ( 4.26 , 2.42 )
;  \draw[  blue, line width = 1.5pt ] ( 4.26 , 2.42 )
-- ( 4.26 , 1.92 )
;  \draw[  blue, line width = 1.5pt ] ( 0 , 1.50 )
-- ( 0.47 , 1.65 )
;  \draw[  blue, line width = 1.5pt ] ( 0.47 , 1.65 )
-- ( 0.47 , 1.15 )
;  \draw[  blue, line width = 1.5pt ] ( 1.89 , 1.63 )
-- ( 1.89 , 2.13 )
( 1.89 , 1.63 )
;  \draw[  blue, line width = 1.5pt ] ( 2.37 , 2.29 )
-- ( 2.84 , 2.44 )
;  \draw[  blue, line width = 1.5pt ] ( 2.84 , 2.44 )
-- ( 3.32 , 2.60 )
;  \draw[  blue, line width = 1.5pt ] ( 3.32 , 2.60 )
-- ( 3.32 , 2.10 )
;  \draw[  blue, line width = 1.5pt ] ( 1.89 , 2.63 )
-- ( 2.37 , 2.79 )
;  \draw[  blue, line width = 1.5pt ] ( 2.37 , 2.79 )
-- ( 2.37 , 2.29 )
;  \draw[  blue, line width = 1.5pt ] ( 1.89 , 2.13 )
-- ( 1.89 , 2.63 )
( 1.89 , 2.13 )
;  \draw[  blue, line width = 1.5pt ] ( 1.30 , -1.08 )
-- ( 0.83 , -1.24 )
;  \draw[  blue, line width = 1.5pt ] ( 1.30 , -1.08 )
-- ( 1.58 , -1.50 )
( 1.30 , -1.08 )
;  \draw[  blue, line width = 1.5pt ] ( 1.58 , -1.50 )
-- ( 1.86 , -1.92 )
( 1.58 , -1.50 )
;  \draw[  blue, line width = 1.5pt ] ( 2.61 , -2.17 )
-- ( 2.13 , -2.33 )
;  \draw[  blue, line width = 1.5pt ] ( 1.86 , -1.92 )
-- ( 2.13 , -2.33 )
( 1.86 , -1.92 )
;  \draw[  blue, line width = 1.5pt ] ( 3.08 , -2.02 )
-- ( 2.61 , -2.17 )
;  \draw[  blue, line width = 1.5pt ] ( 3.56 , -1.86 )
-- ( 3.08 , -2.02 )
;  \draw[  blue, line width = 1.5pt ] ( 4.03 , -1.70 )
-- ( 3.56 , -1.86 )
;  \draw[  blue, line width = 1.5pt ] ( 3.67 , -0.29 )
-- ( 3.95 , -0.71 )
;  \draw[  blue, line width = 1.5pt ] ( 3.95 , -0.71 )
-- ( 4.23 , -1.13 )
;  \draw[  blue, line width = 1.5pt ] ( 4.78 , -1.96 )
-- ( 4.31 , -2.12 )
;  \draw[  blue, line width = 1.5pt ] ( 4.03 , -1.70 )
-- ( 4.31 , -2.12 )
( 4.03 , -1.70 )
;  \draw[  blue, line width = 1.5pt ] ( 3.87 , 0.27 )
-- ( 4.15 , -0.14 )
;  \draw[  blue, line width = 1.5pt ] ( 4.15 , -0.14 )
-- ( 3.67 , -0.29 )
;  \draw[  blue, line width = 1.5pt ] ( 4.23 , -1.13 )
-- ( 4.70 , -0.97 )
( 4.23 , -1.13 )
;  \draw[  blue, line width = 1.5pt ] ( 4.98 , -1.38 )
-- ( 5.26 , -1.80 )
;  \draw[  blue, line width = 1.5pt ] ( 5.26 , -1.80 )
-- ( 4.78 , -1.96 )
;  \draw[  blue, line width = 1.5pt ] ( 4.07 , 0.84 )
-- ( 4.34 , 0.43 )
;  \draw[  blue, line width = 1.5pt ] ( 4.34 , 0.43 )
-- ( 3.87 , 0.27 )
;  \draw[  blue, line width = 1.5pt ] ( 5.45 , -1.23 )
-- ( 4.98 , -1.38 )
;  \draw[  blue, line width = 1.5pt ] ( 4.70 , -0.97 )
-- ( 5.18 , -0.81 )
( 4.70 , -0.97 )
;  \draw[  blue, line width = 1.5pt ] ( 4.54 , 1.00 )
-- ( 4.07 , 0.84 )
;  \draw[  blue, line width = 1.5pt ] ( 5.93 , -1.07 )
-- ( 5.45 , -1.23 )
;  \draw[  blue, line width = 1.5pt ] ( 5.18 , -0.81 )
-- ( 5.65 , -0.65 )
( 5.18 , -0.81 )
;  \draw[  blue, line width = 1.5pt ] ( 4.74 , 1.58 )
-- ( 5.02 , 1.16 )
;  \draw[  blue, line width = 1.5pt ] ( 5.29 , 0.74 )
-- ( 4.82 , 0.59 )
;  \draw[  blue, line width = 1.5pt ] ( 4.54 , 1.00 )
-- ( 4.82 , 0.59 )
( 4.54 , 1.00 )
;  \draw[  blue, line width = 1.5pt ] ( 5.37 , -0.24 )
-- ( 5.65 , -0.65 )
( 5.37 , -0.24 )
;  \draw[  blue, line width = 1.5pt ] ( 5.37 , -0.24 )
-- ( 5.85 , -0.08 )
( 5.37 , -0.24 )
;  \draw[  blue, line width = 1.5pt ] ( 6.40 , -0.91 )
-- ( 5.93 , -1.07 )
;  \draw[  blue, line width = 1.5pt ] ( 5.49 , 1.32 )
-- ( 5.77 , 0.90 )
;  \draw[  blue, line width = 1.5pt ] ( 5.02 , 1.16 )
-- ( 5.49 , 1.32 )
( 5.02 , 1.16 )
;  \draw[  blue, line width = 1.5pt ] ( 5.29 , 0.74 )
-- ( 5.57 , 0.33 )
( 5.29 , 0.74 )
;  \draw[  blue, line width = 1.5pt ] ( 5.57 , 0.33 )
-- ( 5.85 , -0.08 )
( 5.57 , 0.33 )
;  \draw[  blue, line width = 1.5pt ] ( 6.32 , 0.07 )
-- ( 6.60 , -0.34 )
;  \draw[  blue, line width = 1.5pt ] ( 6.60 , -0.34 )
-- ( 6.88 , -0.75 )
;  \draw[  blue, line width = 1.5pt ] ( 6.88 , -0.75 )
-- ( 6.40 , -0.91 )
;  \draw[  blue, line width = 1.5pt ] ( 6.24 , 1.06 )
-- ( 6.52 , 0.64 )
;  \draw[  blue, line width = 1.5pt ] ( 5.77 , 0.90 )
-- ( 6.24 , 1.06 )
( 5.77 , 0.90 )
;  \draw[  blue, line width = 1.5pt ] ( 6.52 , 0.64 )
-- ( 6.80 , 0.23 )
;  \draw[  blue, line width = 1.5pt ] ( 6.80 , 0.23 )
-- ( 6.32 , 0.07 )
;  \draw[  blue, line width = 1.5pt ] ( -0.27 , -1.80 )
-- ( -0.46 , -2.27 )
;  \draw[  blue, line width = 1.5pt ] ( -0.46 , -2.27 )
-- ( -0.74 , -1.85 )
;  \draw[  blue, line width = 1.5pt ] ( 0.36 , -1.29 )
-- ( 0.18 , -1.76 )
;  \draw[  blue, line width = 1.5pt ] ( 0.18 , -1.76 )
-- ( -0.00 , -2.22 )
;  \draw[  blue, line width = 1.5pt ] ( -0.00 , -2.22 )
-- ( -0.27 , -1.80 )
;  \draw[  blue, line width = 1.5pt ] ( 0.83 , -1.24 )
-- ( 0.64 , -1.71 )
;  \draw[  blue, line width = 1.5pt ] ( 0.64 , -1.71 )
-- ( 0.36 , -1.29 )
;  \draw[  blue, line width = 1.5pt ] ( -1.84 , 0.64 )
-- ( -1.66 , 1.10 )
;  \draw[  blue, line width = 1.5pt ] ( -3.32 , 2.21 )
-- ( -3.51 , 1.75 )
( -3.32 , 2.21 )
;  \draw[  blue, line width = 1.5pt ] ( -4.76 , 2.58 )
-- ( -4.57 , 3.05 )
;  \draw[  blue, line width = 1.5pt ] ( -2.03 , 0.18 )
-- ( -1.84 , 0.64 )
;  \draw[  blue, line width = 1.5pt ] ( -3.51 , 1.75 )
-- ( -3.69 , 1.29 )
( -3.51 , 1.75 )
;  \draw[  blue, line width = 1.5pt ] ( -4.94 , 2.12 )
-- ( -4.76 , 2.58 )
;  \draw[  blue, line width = 1.5pt ] ( -1.80 , -0.56 )
-- ( -2.22 , -0.28 )
;  \draw[  blue, line width = 1.5pt ] ( -2.22 , -0.28 )
-- ( -2.03 , 0.18 )
;  \draw[  blue, line width = 1.5pt ] ( -3.88 , 0.82 )
-- ( -4.30 , 1.10 )
;  \draw[  blue, line width = 1.5pt ] ( -3.69 , 1.29 )
-- ( -3.88 , 0.82 )
( -3.69 , 1.29 )
;  \draw[  blue, line width = 1.5pt ] ( -5.13 , 1.65 )
-- ( -4.94 , 2.12 )
;  \draw[  blue, line width = 1.5pt ] ( -0.74 , -1.85 )
-- ( -1.15 , -1.57 )
;  \draw[  blue, line width = 1.5pt ] ( -1.57 , -1.30 )
-- ( -1.99 , -1.02 )
;  \draw[  blue, line width = 1.5pt ] ( -1.99 , -1.02 )
-- ( -1.80 , -0.56 )
;  \draw[  blue, line width = 1.5pt ] ( -4.48 , 0.63 )
-- ( -4.90 , 0.91 )
;  \draw[  blue, line width = 1.5pt ] ( -4.30 , 1.10 )
-- ( -4.48 , 0.63 )
( -4.30 , 1.10 )
;  \draw[  blue, line width = 1.5pt ] ( -4.90 , 0.91 )
-- ( -5.31 , 1.19 )
;  \draw[  blue, line width = 1.5pt ] ( -5.31 , 1.19 )
-- ( -5.13 , 1.65 )
;  \draw[  blue, line width = 1.5pt ] ( -1.34 , -2.04 )
-- ( -1.76 , -1.76 )
;  \draw[  blue, line width = 1.5pt ] ( -1.76 , -1.76 )
-- ( -1.57 , -1.30 )
;  \draw[  blue, line width = 1.5pt ] ( -1.15 , -1.57 )
-- ( -1.34 , -2.04 )
( -1.15 , -1.57 )
;  \draw[  blue, line width = 1.5pt ] ( -0.41 , 1.77 )
-- ( 0 , 1.50 )
;  \draw[  blue, line width = 1.5pt ] ( -0.83 , 2.05 )
-- ( -0.41 , 1.77 )
;  \draw[  blue, line width = 1.5pt ] ( -1.24 , 1.83 )
-- ( -1.24 , 2.33 )
;  \draw[  blue, line width = 1.5pt ] ( -1.24 , 2.33 )
-- ( -0.83 , 2.05 )
;  \draw[  blue, line width = 1.5pt ] ( -1.66 , 1.10 )
-- ( -1.66 , 1.60 )
;  \draw[  blue, line width = 1.5pt ] ( -1.66 , 1.60 )
-- ( -1.66 , 2.10 )
;  \draw[  blue, line width = 1.5pt ] ( -1.66 , 2.10 )
-- ( -1.24 , 1.83 )
;  \draw[  blue, line width = 1.5pt ] ( -3.74 , 2.99 )
-- ( -3.32 , 2.71 )
;  \draw[  blue, line width = 1.5pt ] ( -3.32 , 2.21 )
-- ( -3.32 , 2.71 )
( -3.32 , 2.21 )
;  \draw[  blue, line width = 1.5pt ] ( -4.16 , 3.27 )
-- ( -3.74 , 2.99 )
;  \draw[  blue, line width = 1.5pt ] ( -4.57 , 3.05 )
-- ( -4.57 , 3.55 )
;  \draw[  blue, line width = 1.5pt ] ( -4.57 , 3.55 )
-- ( -4.16 , 3.27 )
;
